An Overview of Structural Coverage Metrics for Testing Neural Networks

Deep neural network (DNN) models, including those used in safety-critical domains, need to be thoroughly tested to ensure that they can reliably perform well in different scenarios. In this article, we provide an overview of structural coverage metrics for testing DNN models, including neuron coverage (NC), k-multisection neuron coverage (kMNC), top-k neuron coverage (TKNC), neuron boundary coverage (NBC), strong neuron activation coverage (SNAC) and modified condition/decision coverage (MC/DC). We evaluate the metrics on realistic DNN models used for perception tasks (including LeNet-1, LeNet-4, LeNet-5, and ResNet20) as well as on networks used in autonomy (TaxiNet). We also provide a tool, DNNCov, which can measure the testing coverage for all these metrics. DNNCov outputs an informative coverage report to enable researchers and practitioners to assess the adequacy of DNN testing, compare different coverage measures, and to more conveniently inspect the model's internals during testing.

==> tables/quantitative/adversarial0.01.tex <==



\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Adversarial 0.01}
\label{tab:quantitative-adversarial0.01}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&246.40&0.80&0.80&232.00&246.00&252.20&244.80&0.00&98,840.40&125,897.80&199,146.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.66&94.57&55.21&0.00&749.13&20,325.60&35,183.88\\
&Std.&78.73&1.42&33.36&6.42&0.02&0.03&40.92&61.28&73.75&71.70&0.00&7,946.83&40,408.32&44,938.10\\
&Var.&6,198.64&2.03&1,112.89&41.19&0.00&0.00&1,674.34&3,755.88&5,440.95&5,143.82&0.00&63,197,042.79&1,633,247,596.37&2,019,902,359.70\\\hline
\multirow{5}{*}{Adversarial (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&13.00&243.60&246.00&0.80&0.80&232.00&245.60&251.20&246.00&0.00&99,051.40&125,884.40&199,491.20\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.22&94.56&55.50&0.00&750.78&20,319.80&35,147.82\\
&Std.&78.74&1.42&33.36&6.42&0.02&0.03&40.96&61.80&73.73&72.03&0.00&7,966.20&40,394.70&44,894.35\\
&Var.&6,200.70&2.03&1,113.18&41.20&0.00&0.00&1,677.25&3,820.56&5,438.45&5,190.63&0.00&63,508,493.73&1,632,233,481.23&2,016,103,470.61\\\hline
\multirow{5}{*}{Adversarial (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.60&247.80&0.80&0.80&232.00&246.60&252.00&245.80&0.00&98,907.80&125,735.80&198,580.80\\
&Avg&74.40&0.99&14.98&0.94&0.00&0.00&218.81&196.81&94.00&55.53&0.00&747.93&20,290.02&35,131.31\\
&Std.&78.87&1.43&33.37&6.42&0.02&0.03&40.98&61.11&73.49&72.06&0.00&7,938.27&40,346.93&44,864.90\\
&Var.&6,220.12&2.03&1,113.87&41.21&0.00&0.00&1,679.37&3,735.26&5,401.73&5,195.07&0.00&63,051,574.12&1,628,385,973.21&2,013,505,910.20\\\hline
\multirow{5}{*}{Adversarial (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.40&239.60&247.40&0.80&0.80&232.00&246.00&251.20&245.60&0.00&99,376.00&125,870.60&199,401.60\\
&Avg&74.08&0.99&14.94&0.94&0.00&0.00&218.81&196.59&94.77&55.35&0.00&750.51&20,359.66&35,233.70\\
&Std.&78.57&1.42&33.23&6.41&0.02&0.03&41.06&61.33&73.79&71.88&0.00&7,963.04&40,471.21&45,018.02\\
&Var.&6,173.73&2.03&1,105.01&41.18&0.00&0.00&1,685.59&3,763.67&5,446.85&5,170.27&0.00&63,449,045.92&1,638,370,269.99&2,027,103,571.77\\\hline
\multirow{5}{*}{Adversarial (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.80&243.40&246.80&1.00&1.00&232.00&246.20&252.60&247.60&0.00&98,053.80&126,631.20&199,482.20\\
&Avg&74.46&0.99&14.98&0.94&0.00&0.00&218.81&196.39&94.99&56.07&0.00&743.97&20,388.69&35,357.64\\
&Std.&78.86&1.42&33.39&6.42&0.03&0.03&40.99&61.49&73.77&72.67&0.00&7,893.35&40,537.40&45,176.01\\
&Var.&6,217.96&2.03&1,115.40&41.17&0.00&0.00&1,679.92&3,780.55&5,443.77&5,282.03&0.00&62,330,839.26&1,643,880,038.28&2,041,477,612.30\\\hline
\multirow{5}{*}{Adversarial (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.00&245.40&247.60&0.80&0.80&232.00&245.60&251.60&244.40&0.00&99,353.60&126,512.60&199,092.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.41&93.22&55.40&0.00&749.01&20,325.00&35,200.26\\
&Std.&78.80&1.42&33.44&6.42&0.02&0.03&41.00&61.51&73.45&72.05&0.00&7,964.38&40,438.32&44,987.93\\
&Var.&6,210.14&2.03&1,118.40&41.26&0.00&0.00&1,681.01&3,785.39&5,395.49&5,193.77&0.00&63,474,745.53&1,635,615,279.61&2,024,402,032.03\\\hline
\multirow{5}{*}{Adversarial (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&245.00&0.80&0.80&232.00&248.60&252.60&252.40&0.00&100,016.60&125,901.00&199,081.40\\
&Avg&74.39&0.99&14.98&0.94&0.00&0.00&218.81&196.63&95.85&56.13&0.00&752.76&20,348.35&35,270.03\\
&Std.&78.82&1.42&33.39&6.42&0.03&0.04&40.89&61.23&73.65&72.94&0.00&7,998.60&40,470.75&45,032.15\\
&Var.&6,213.51&2.03&1,115.04&41.17&0.00&0.00&1,671.81&3,748.70&5,424.76&5,320.21&0.00&63,989,837.24&1,638,136,362.75&2,028,186,101.38\\\hline
\end{tabular}
}
\end{table*}


==> tables/quantitative/adversarial0.05.tex <==


\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Adversarial 0.05}
\label{tab:quantitative-adversarial0.05}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&246.40&0.80&0.80&232.00&246.00&252.20&244.80&0.00&98,840.40&125,897.80&199,146.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.66&94.57&55.21&0.00&749.13&20,325.60&35,183.88\\
&Std.&78.73&1.42&33.36&6.42&0.02&0.03&40.92&61.28&73.75&71.70&0.00&7,946.83&40,408.32&44,938.10\\
&Var.&6,198.64&2.03&1,112.89&41.19&0.00&0.00&1,674.34&3,755.88&5,440.95&5,143.82&0.00&63,197,042.79&1,633,247,596.37&2,019,902,359.70\\\hline
\multirow{5}{*}{Adversarial (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.60&243.80&247.40&1.40&1.40&232.00&245.00&251.80&243.20&0.00&99,046.60&126,548.00&200,341.80\\
&Avg&74.43&0.99&14.98&0.94&0.00&0.00&218.81&196.71&94.62&55.30&0.00&750.96&20,395.97&35,458.18\\
&Std.&78.84&1.42&33.34&6.42&0.05&0.06&40.95&61.17&73.77&71.82&0.00&7,960.28&40,560.88&45,322.25\\
&Var.&6,216.11&2.03&1,112.09&41.27&0.00&0.00&1,676.74&3,741.38&5,444.11&5,160.31&0.00&63,425,820.87&1,645,481,948.24&2,054,369,861.41\\\hline
\multirow{5}{*}{Adversarial (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.40&242.40&245.60&1.20&1.20&232.00&246.40&251.40&245.80&0.00&98,755.80&126,715.80&200,541.00\\
&Avg&74.32&0.99&14.98&0.94&0.00&0.00&218.81&196.81&93.94&55.58&0.00&749.84&20,405.93&35,540.45\\
&Std.&78.70&1.42&33.33&6.41&0.05&0.06&40.89&61.06&73.44&72.16&0.00&7,944.03&40,589.58&45,435.46\\
&Var.&6,193.98&2.03&1,111.05&41.13&0.00&0.00&1,672.49&3,729.49&5,394.50&5,209.66&0.00&63,150,014.54&1,648,096,802.86&2,065,220,408.92\\\hline
\multirow{5}{*}{Adversarial (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.60&247.20&1.40&1.40&232.00&245.00&250.40&245.40&0.00&100,500.20&127,709.80&203,231.20\\
&Avg&74.77&0.99&14.98&0.94&0.00&0.00&218.81&196.89&94.64&55.85&0.00&758.75&20,652.14&36,083.20\\
&Std.&78.96&1.42&33.28&6.42&0.05&0.08&40.86&60.95&73.86&72.41&0.00&8,025.96&41,081.81&46,165.40\\
&Var.&6,234.44&2.02&1,107.90&41.19&0.00&0.00&1,669.22&3,715.04&5,457.91&5,245.42&0.00&64,445,327.53&1,688,121,072.92&2,131,526,529.28\\\hline
\multirow{5}{*}{Adversarial (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.20&241.80&243.80&2.00&2.00&232.00&247.60&252.00&247.80&0.00&100,255.60&129,590.20&205,228.40\\
&Avg&74.98&0.99&14.98&0.94&0.00&0.01&218.81&196.87&94.68&55.54&0.00&754.05&20,676.13&36,373.85\\
&Std.&79.11&1.42&33.28&6.42&0.07&0.10&40.92&61.07&74.34&72.16&0.00&7,984.34&41,162.00&46,680.11\\
&Var.&6,258.54&2.02&1,107.78&41.21&0.01&0.01&1,674.51&3,729.56&5,527.93&5,208.78&0.00&63,823,354.99&1,694,688,936.45&2,179,377,593.20\\\hline
\multirow{5}{*}{Adversarial (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.20&241.60&249.20&2.40&2.40&232.00&246.80&250.40&245.00&0.00&100,525.20&129,394.40&206,095.20\\
&Avg&75.01&0.99&14.98&0.94&0.00&0.01&218.81&197.74&93.72&55.73&0.00&761.63&20,814.14&36,851.64\\
&Std.&79.01&1.41&33.22&6.41&0.09&0.12&41.01&59.82&73.32&72.55&0.00&8,053.26&41,422.88&47,293.07\\
&Var.&6,242.23&2.01&1,103.69&41.17&0.01&0.02&1,681.39&3,579.26&5,377.00&5,266.99&0.00&64,920,959.57&1,716,057,909.76&2,236,834,512.65\\\hline
\multirow{5}{*}{Adversarial (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.00&243.80&247.60&1.80&1.80&232.00&246.00&253.60&250.60&0.00&101,140.80&130,800.20&208,427.40\\
&Avg&75.28&0.99&14.98&0.94&0.01&0.01&218.81&196.91&95.75&56.57&0.00&764.98&20,985.98&37,337.72\\
&Std.&79.16&1.42&33.17&6.41&0.09&0.13&41.11&60.64&74.19&73.57&0.00&8,091.36&41,774.54&48,043.28\\
&Var.&6,267.09&2.01&1,100.66&41.11&0.01&0.02&1,690.37&3,677.76&5,505.81&5,412.91&0.00&65,507,616.31&1,745,459,091.85&2,308,414,385.40\\\hline
\end{tabular}
}
\end{table*}

==> tables/quantitative/adversarial0.10.tex <==


\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Adversarial 0.10}
\label{tab:quantitative-adversarial0.10}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&246.40&0.80&0.80&232.00&246.00&252.20&244.80&0.00&98,840.40&125,897.80&199,146.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.66&94.57&55.21&0.00&749.13&20,325.60&35,183.88\\
&Std.&78.73&1.42&33.36&6.42&0.02&0.03&40.92&61.28&73.75&71.70&0.00&7,946.83&40,408.32&44,938.10\\
&Var.&6,198.64&2.03&1,112.89&41.19&0.00&0.00&1,674.34&3,755.88&5,440.95&5,143.82&0.00&63,197,042.79&1,633,247,596.37&2,019,902,359.70\\\hline
\multirow{5}{*}{Adversarial (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.00&246.40&3.80&3.80&232.00&246.20&251.00&244.40&0.00&99,533.40&127,342.60&201,300.60\\
&Avg&74.40&0.99&14.98&0.94&0.01&0.02&218.81&196.95&94.33&55.21&0.00&755.57&20,519.41&35,912.81\\
&Std.&78.63&1.42&33.31&6.41&0.15&0.21&40.89&60.69&73.67&71.76&0.00&8,009.00&40,787.60&45,940.49\\
&Var.&6,182.49&2.02&1,109.82&41.11&0.02&0.05&1,672.08&3,695.40&5,429.43&5,152.79&0.00&64,179,895.60&1,664,006,378.45&2,110,961,351.69\\\hline
\multirow{5}{*}{Adversarial (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.00&242.00&246.20&5.40&5.40&232.00&244.80&251.60&242.40&0.00&100,111.20&129,369.60&205,544.20\\
&Avg&75.22&0.99&14.98&0.94&0.02&0.03&218.81&196.67&94.60&55.28&0.00&756.86&20,677.33&36,563.66\\
&Std.&78.96&1.42&33.27&6.41&0.20&0.29&40.85&60.94&73.85&71.71&0.00&7,998.49&41,120.50&46,861.67\\
&Var.&6,235.01&2.01&1,107.23&41.10&0.04&0.08&1,668.65&3,713.39&5,455.79&5,145.66&0.00&64,017,678.53&1,691,272,081.04&2,196,356,891.03\\\hline
\multirow{5}{*}{Adversarial (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.00&242.40&246.60&7.00&7.00&232.00&247.80&252.40&247.20&0.00&99,714.40&131,324.80&210,128.40\\
&Avg&75.45&0.99&14.98&0.94&0.02&0.05&218.81&196.50&94.55&55.84&0.00&758.52&20,993.85&37,370.93\\
&Std.&78.87&1.41&33.14&6.40&0.28&0.40&40.88&60.97&74.07&72.30&0.00&7,972.98&41,752.63&47,988.15\\
&Var.&6,220.43&2.00&1,098.76&40.96&0.09&0.17&1,671.35&3,717.35&5,489.13&5,229.25&0.00&63,627,849.45&1,743,664,326.54&2,303,206,368.90\\\hline
\multirow{5}{*}{Adversarial (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.20&241.60&244.40&14.20&14.20&232.00&247.60&252.40&244.80&0.00&103,628.20&134,507.80&217,061.40\\
&Avg&76.26&0.99&14.98&0.94&0.05&0.09&218.81&196.71&94.42&55.87&0.00&779.02&21,358.64&38,804.50\\
&Std.&78.97&1.40&33.05&6.39&0.54&0.76&40.68&60.44&73.93&72.52&0.00&8,169.55&42,505.87&50,073.39\\
&Var.&6,236.77&1.98&1,092.38&40.76&0.30&0.60&1,654.81&3,655.62&5,467.46&5,260.46&0.00&66,780,104.15&1,807,013,205.85&2,507,627,130.23\\\hline
\multirow{5}{*}{Adversarial (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.20&235.00&247.60&21.00&21.00&232.00&246.20&252.60&243.40&0.00&106,533.00&138,700.60&226,584.00\\
&Avg&77.21&0.98&14.91&0.94&0.07&0.14&218.81&196.39&93.97&55.21&0.00&789.34&21,733.24&40,228.64\\
&Std.&79.13&1.40&32.73&6.37&0.76&1.07&40.79&60.66&73.85&71.77&0.00&8,260.06&43,328.82&52,279.91\\
&Var.&6,261.81&1.96&1,071.03&40.63&0.58&1.15&1,664.25&3,680.02&5,457.79&5,151.68&0.00&68,267,269.24&1,877,726,824.64&2,733,615,255.28\\\hline
\multirow{5}{*}{Adversarial (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.60&233.40&240.20&25.40&25.40&232.00&248.20&253.80&249.20&0.00&106,929.60&142,408.20&234,034.20\\
&Avg&78.44&0.98&14.91&0.94&0.09&0.18&218.81&196.66&94.14&56.54&0.00&794.13&22,246.70&41,912.78\\
&Std.&79.39&1.39&32.58&6.34&1.00&1.41&40.78&59.57&74.25&73.43&0.00&8,302.24&44,400.16&54,887.79\\
&Var.&6,302.98&1.94&1,061.47&40.26&1.01&1.99&1,662.86&3,551.81&5,513.48&5,394.16&0.00&69,025,360.87&1,971,891,928.32&3,013,303,512.27\\\hline
\end{tabular}
}
\end{table*}

==> tables/quantitative/adversarial0.20.tex <==


\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Adversarial 0.20}
\label{tab:quantitative-adversarial0.20}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&246.40&0.80&0.80&232.00&246.00&252.20&244.80&0.00&98,840.40&125,897.80&199,146.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.66&94.57&55.21&0.00&749.13&20,325.60&35,183.88\\
&Std.&78.73&1.42&33.36&6.42&0.02&0.03&40.92&61.28&73.75&71.70&0.00&7,946.83&40,408.32&44,938.10\\
&Var.&6,198.64&2.03&1,112.89&41.19&0.00&0.00&1,674.34&3,755.88&5,440.95&5,143.82&0.00&63,197,042.79&1,633,247,596.37&2,019,902,359.70\\\hline
\multirow{5}{*}{Adversarial (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&244.00&247.00&7.80&7.80&232.00&245.80&252.00&245.40&0.00&99,085.20&128,370.80&203,798.20\\
&Avg&74.85&0.99&14.98&0.94&0.04&0.09&218.81&196.66&95.19&55.18&0.00&757.07&20,573.16&36,236.93\\
&Std.&78.76&1.42&33.21&6.40&0.42&0.58&40.76&60.94&74.06&71.70&0.00&7,964.02&40,877.38&46,360.48\\
&Var.&6,202.52&2.02&1,103.27&40.99&0.17&0.35&1,661.20&3,713.62&5,488.11&5,144.42&0.00&63,470,847.38&1,671,421,409.96&2,151,743,467.02\\\hline
\multirow{5}{*}{Adversarial (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&239.40&248.60&14.80&14.80&232.00&247.40&252.20&244.00&102.80&99,566.20&130,171.40&208,778.60\\
&Avg&75.41&0.98&14.91&0.94&0.07&0.13&218.81&196.85&94.44&55.08&0.19&766.17&20,818.92&37,225.58\\
&Std.&78.80&1.41&32.89&6.37&0.66&0.93&40.78&60.32&73.69&71.64&4.44&7,999.02&41,369.23&47,775.39\\
&Var.&6,209.84&2.00&1,082.00&40.63&0.45&0.89&1,663.04&3,639.02&5,432.57&5,134.62&98.40&50,935,470.33&1,711,669,276.42&2,282,788,725.14\\\hline
\multirow{5}{*}{Adversarial (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.00&244.00&251.00&22.00&22.00&232.00&248.40&253.00&246.20&397.20&101,193.60&132,889.20&213,432.60\\
&Avg&76.05&0.98&14.98&0.94&0.12&0.23&218.81&196.74&93.61&55.44&0.87&778.01&21,112.71&38,382.49\\
&Std.&78.92&1.41&33.00&6.38&1.08&1.51&40.64&60.09&73.49&71.96&17.92&8,045.42&41,929.14&49,409.35\\
&Var.&6,228.09&1.98&1,089.56&40.62&1.18&2.32&1,651.82&3,611.81&5,404.27&5,180.05&557.47&64,785,385.94&1,758,560,214.72&2,441,890,620.89\\\hline
\multirow{5}{*}{Adversarial (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.00&240.60&248.00&35.60&35.60&232.00&243.00&251.20&248.40&320.60&104,813.40&137,620.00&225,675.60\\
&Avg&77.29&0.98&14.91&0.94&0.17&0.34&218.81&195.86&94.41&55.78&0.60&794.48&21,652.68&40,348.78\\
&Std.&78.91&1.40&32.58&6.33&1.64&2.31&40.43&60.61&73.72&72.52&13.84&8,143.48&43,043.76&52,330.50\\
&Var.&6,227.94&1.95&1,061.77&40.04&2.70&5.35&1,634.97&3,677.50&5,438.00&5,261.08&207.49&66,360,472.50&1,853,138,304.03&2,738,957,290.24\\\hline
\multirow{5}{*}{Adversarial (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&239.80&243.40&52.60&52.60&232.00&253.40&249.40&251.40&840.00&105,458.80&141,215.80&232,521.20\\
&Avg&78.27&0.98&14.91&0.94&0.26&0.51&218.81&195.89&93.02&55.52&2.40&818.27&22,184.44&42,585.93\\
&Std.&78.79&1.39&32.42&6.29&2.40&3.38&40.31&60.04&73.21&72.23&42.93&8,266.97&44,067.54&55,574.02\\
&Var.&6,208.15&1.92&1,051.17&39.56&5.79&11.46&1,624.74&3,606.03&5,362.71&5,217.29&2,085.84&68,349,634.49&1,942,252,693.96&3,088,826,594.80\\\hline
\multirow{5}{*}{Adversarial (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&11.80&236.20&246.60&76.40&76.40&232.00&250.80&252.40&245.00&1,188.00&112,392.80&147,373.00&247,189.20\\
&Avg&80.29&0.98&14.91&0.94&0.38&0.76&218.81&195.17&94.28&55.59&2.82&852.52&22,745.32&45,048.35\\
&Std.&78.94&1.37&32.12&6.27&3.56&5.01&39.92&60.19&74.18&72.43&55.06&8,479.84&45,338.01&59,664.75\\
&Var.&6,231.74&1.88&1,031.93&39.25&12.69&25.09&1,593.66&3,622.74&5,505.84&5,246.43&3,336.42&71,948,612.40&2,056,068,161.01&3,560,458,918.46\\\hline
\end{tabular}
}
\end{table*}

==> tables/quantitative/adversarial0.30.tex <==


\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Adversarial 0.30}
\label{tab:quantitative-adversarial0.30}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&243.80&246.40&0.80&0.80&232.00&246.00&252.20&244.80&0.00&98,840.40&125,897.80&199,146.00\\
&Avg&74.26&0.99&14.98&0.94&0.00&0.00&218.81&196.66&94.57&55.21&0.00&749.13&20,325.60&35,183.88\\
&Std.&78.73&1.42&33.36&6.42&0.02&0.03&40.92&61.28&73.75&71.70&0.00&7,946.83&40,408.32&44,938.10\\
&Var.&6,198.64&2.03&1,112.89&41.19&0.00&0.00&1,674.34&3,755.88&5,440.95&5,143.82&0.00&63,197,042.79&1,633,247,596.37&2,019,902,359.70\\\hline
\multirow{5}{*}{Adversarial (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&254.80&12.60&244.40&246.60&6.80&6.80&232.00&244.40&250.60&245.00&232.60&98,260.60&127,937.60&203,045.00\\
&Avg&74.62&0.99&14.98&0.94&0.03&0.07&218.81&196.21&93.34&55.24&0.46&755.49&20,578.96&36,211.28\\
&Std.&78.60&1.42&95.82&6.40&0.34&0.47&40.81&61.33&73.26&71.75&10.07&7,911.47&40,888.24&46,344.78\\
&Var.&6,178.46&2.01&1,104.04&40.93&0.11&0.22&1,665.75&3,762.31&5,368.85&5,150.71&208.82&62,640,337.45&1,672,313,012.50&2,148,389,038.52\\\hline
\multirow{5}{*}{Adversarial (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.40&239.20&245.20&15.20&15.20&232.00&247.00&250.60&250.40&602.80&96,876.00&130,198.40&206,618.20\\
&Avg&75.28&0.98&14.91&0.94&0.08&0.15&218.81&196.74&93.60&55.87&1.35&760.03&20,794.76&37,188.93\\
&Std.&78.67&1.41&32.83&6.37&0.72&1.01&40.71&60.43&73.59&72.34&28.03&7,835.01&41,300.57&47,706.59\\
&Var.&6,189.04&2.00&1,077.60&40.54&0.52&1.02&1,657.32&3,651.28&5,417.07&5,235.11&828.03&61,421,918.11&1,706,168,559.46&2,276,461,198.09\\\hline
\multirow{5}{*}{Adversarial (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&12.60&239.00&248.80&22.40&22.40&232.00&249.20&251.00&247.40&935.00&98,321.60&133,099.20&212,332.80\\
&Avg&76.33&0.98&14.91&0.94&0.11&0.23&218.81&196.54&93.74&55.89&1.97&773.12&21,110.53&38,326.19\\
&Std.&79.00&1.41&32.71&6.35&1.08&1.51&40.51&60.26&73.42&72.45&42.45&7,884.19&41,925.11&49,322.04\\
&Var.&6,241.61&1.98&1,069.82&40.34&1.17&2.31&1,640.62&3,631.34&5,392.80&5,250.99&2,062.30&62,223,985.00&1,757,959,520.17&2,432,847,799.95\\\hline
\multirow{5}{*}{Adversarial (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&11.60&238.00&249.40&33.20&33.20&232.00&250.40&251.00&248.60&981.80&97,635.00&137,262.00&222,595.00\\
&Avg&77.74&0.98&14.91&0.94&0.17&0.34&218.81&196.04&95.02&56.05&2.31&777.44&21,598.17&40,267.24\\
&Std.&79.04&1.39&32.42&6.31&1.61&2.26&40.46&60.42&73.83&72.73&44.85&7,745.57&42,925.26&52,162.78\\
&Var.&6,247.64&1.95&1,050.90&39.85&2.59&5.12&1,637.02&3,652.64&5,454.03&5,289.68&2,446.49&60,078,790.23&1,842,851,431.49&2,721,331,827.01\\\hline
\multirow{5}{*}{Adversarial (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&11.60&235.80&247.40&45.20&45.20&232.00&250.60&250.00&246.60&1,734.60&97,389.00&141,170.20&230,062.80\\
&Avg&78.61&0.98&14.91&0.94&0.24&0.48&1,218.81&195.20&92.92&55.85&4.15&788.27&22,011.75&41,959.93\\
&Std.&78.74&1.38&32.21&6.28&2.19&3.07&40.15&60.82&73.25&72.57&80.07&7,666.96&43,777.69&54,783.94\\
&Var.&6,200.31&1.91&1,037.72&39.48&4.84&9.56&1,612.15&3,700.53&5,367.98&5,266.52&6,868.04&58,927,033.66&1,917,065,786.65&3,001,816,353.08\\\hline
\multirow{5}{*}{Adversarial (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
&Max&255.00&11.60&233.00&247.20&69.20&69.20&232.00&251.60&253.40&246.60&2,363.60&95,831.60&146,695.20&242,320.40\\
&Avg&80.15&0.98&14.91&0.94&0.34&0.68&218.81&194.41&93.05&56.35&6.08&797.94&22,522.68&44,255.64\\
&Std.&78.65&1.37&32.04&6.25&3.17&4.46&39.96&60.96&73.37&73.38&114.16&7,496.02&44,955.50&58,645.70\\
&Var.&6,184.81&1.88&1,026.34&39.04&10.10&19.96&1,596.77&3,717.62&5,384.96&5,386.06&13,825.67&56,250,911.82&2,021,423,808.66&3,439,790,761.82\\\hline
\end{tabular}
}
\end{table*}

==> tables/quantitative/functional.tex <==




\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Functional Diversity}
\label{tab:quantitative-functional}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{1 Label} &Min&0.00&0.00&0.00&0.00&0.00&0.00&2.80&0.00&0.00&0.00&0.00&0.00&0.00&216.20\\
&Max&254.60&16.00&245.60&245.60&0.80&0.80&251.00&251.40&253.40&250.40&0.00&0.00&47,428.40&80,757.40\\
&Avg&44.26&0.80&9.96&0.74&0.00&0.00&40.91&64.62&85.99&42.92&0.00&0.00&14,994.11&15,958.12\\
&Std.&67.43&1.67&28.09&4.80&0.02&0.03&41.07&67.64&82.06&63.53&0.00&0.00&14,461.88&18,205.57\\
&Var.&4,546.93&2.81&789.82&23.07&0.00&0.00&1,701.20&4,622.98&6,738.52&4,056.32&0.00&0.00&217,047,915.68&343,441,740.25\\\hline
\multirow{5}{*}{2 Label}&Min&0.00&0.00&0.00&0.00&0.00&0.00&4.00&0.00&0.00&0.00&0.00&0.00&0.00&1,477.60\\
&Max&254.40&15.80&248.40&248.40&0.80&0.80&243.40&252.20&253.80&251.20&0.00&0.00&97,258.20&133,238.20\\
&Avg&60.94&0.80&10.75&0.74&0.00&0.00&39.18&64.96&103.59&61.32&0.00&0.00&35,909.95&34,961.83\\
&Std.&73.76&1.41&27.19&4.42&0.02&0.03&37.41&71.45&83.24&72.14&0.00&0.00&28,981.19&32,381.83\\
&Var.&5,448.96&2.00&739.77&19.55&0.00&0.00&1,438.19&5,115.34&6,929.62&5,221.87&0.00&0.00&876,336,576.54&948,267,269.32\\\hline
\multirow{5}{*}{3 Label}&Min&0.00&0.00&0.00&0.00&0.00&0.00&4.20&0.00&0.00&0.00&0.00&0.00&0.00&1,938.00\\
&Max&254.60&13.00&247.80&247.80&1.00&1.00&246.20&254.40&253.80&252.60&0.00&0.00&79,038.00&123,038.00\\
&Avg&62.56&0.80&10.75&0.74&0.00&0.00&40.57&74.05&107.34&69.80&0.00&0.00&33,527.10&32,330.26\\
&Std.&75.06&1.35&26.61&4.30&0.02&0.03&40.88&78.58&82.74&74.80&0.00&0.00&24,514.47&28,511.28\\
&Var.&5,633.95&1.81&708.49&18.46&0.00&0.00&1,653.55&6,176.56&6,857.19&5,597.32&0.00&0.00&626,138,662.98&846,297,103.12\\\hline
\multirow{5}{*}{5 Label}&Min&0.00&0.00&0.00&0.00&0.00&0.00&5.40&0.00&0.00&0.00&0.00&0.00&0.00&4,522.60\\
&Max&254.80&12.40&225.00&231.60&0.60&0.60&251.60&253.80&254.00&249.20&0.00&0.00&99,603.80&150,463.80\\
&Avg&67.10&0.80&11.20&0.75&0.00&0.00&40.91&72.08&110.00&82.96&0.00&0.00&46,368.74&42,574.60\\
&Std.&74.00&1.29&25.64&4.17&0.02&0.02&41.45&78.63&81.34&77.60&0.00&0.00&31,107.93&36,329.81\\
&Var.&5,481.07&1.66&658.21&17.35&0.00&0.00&1,735.10&6,191.04&6,628.71&6,022.57&0.00&0.00&978,054,306.10&1,339,090,207.71\\\hline
\multirow{5}{*}{7 Label}&Min&0.00&0.00&0.00&0.00&0.00&0.00&5.40&0.00&0.00&0.00&0.00&0.00&0.00&6,134.00\\
&Max&254.80&11.80&245.60&245.60&1.00&1.00&246.40&254.60&254.20&251.00&0.00&0.00&94,130.20&150,946.20\\
&Avg&69.72&0.80&11.27&0.75&0.00&0.00&41.26&73.64&113.12&79.15&0.00&0.00&45,791.54&42,525.83\\
&Std.&75.85&1.26&25.21&4.10&0.02&0.03&43.17&79.22&80.76&74.10&0.00&0.00&29,717.48&35,590.58\\
&Var.&5,753.85&1.59&635.47&16.80&0.00&0.00&1,869.37&6,277.48&6,525.08&5,493.58&0.00&0.00&736,984,671.60&1,267,964,398.52\\\hline
\multirow{5}{*}{10 Label}&Min&0.00&0.00&0.00&0.00&0.00&0.00&3.20&0.00&0.00&0.00&0.00&0.00&0.00&7,972.00\\
&Max&254.80&10.80&228.80&228.80&0.80&0.80&246.80&254.40&253.80&252.60&0.00&0.00&90,890.80&142,748.00\\
&Avg&72.01&0.80&11.23&0.75&0.00&0.00&39.53&80.42&110.70&80.85&0.00&0.00&44,167.25&40,287.12\\
&Std.&76.94&1.25&24.34&4.01&0.02&0.03&39.64&83.46&81.18&75.04&0.00&0.00&28,187.31&32,664.23\\
&Var.&5,919.58&1.55&592.63&16.11&0.00&0.00&1,573.37&6,967.05&6,590.26&5,630.99&0.00&0.00&795,678,292.52&1,069,718,510.41\\\hline
\end{tabular}
}
\end{table*}


==> tables/quantitative/poisoned.tex <==


\begin{table*}[t]
	\centering
	\caption{Quantitative Information for Poisoned}
\label{tab:quantitative-poisoned}
\scalebox{0.6}{\begin{tabular}{|C{2.2cm}|C{0.8cm}|R{1.5cm}|R{1.7cm}|R{1.5cm}|R{1.5cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{1.3cm}|R{2.0cm}|R{2.0cm}|R{2.0cm}|}
		 \hline
		   	    \textbf{Dataset}  &  \textbf{Metric}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
\multirow{5}{*}{Clean} &Min&0.00&0.00&0.00&0.00&0.00&0.00&30.80&0.00&0.00&0.00&0.00&0.00&0.00&12,986.40\\
&Max&255.00&12.60&247.00&250.20&1.00&1.00&232.60&247.40&253.80&248.20&0.00&156,211.40&166,161.00&219,296.00\\
&Avg&65.99&1.00&15.84&0.95&0.00&0.00&221.60&199.85&122.49&99.68&0.00&882.18&66,915.34&43,847.31\\
&Std.&74.18&1.49&33.46&5.05&0.03&0.03&32.65&56.13&77.95&73.52&0.00&10,372.68&38,601.23&31,083.70\\
&Var.&5,503.32&2.21&1,120.00&25.46&0.00&0.00&1,071.57&3,151.56&6,076.93&5,405.70&0.00&107,599,179.64&1,490,070,791.53&966,466,131.37\\\hline
\multirow{5}{*}{Poisoned (1\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&36.80&0.00&0.00&0.00&0.00&0.00&0.00&13,143.20\\
&Max&255.00&12.60&246.40&249.60&7.20&7.20&236.80&244.00&253.60&250.00&0.00&156,178.60&166,131.00&219,090.40\\
&Avg&66.05&1.00&15.84&0.95&0.00&0.01&221.95&199.66&122.05&98.81&0.00&882.20&67,037.18&43,973.12\\
&Std.&74.17&1.49&33.43&5.04&0.13&0.19&31.73&56.21&78.03&73.32&0.00&10,372.88&38,651.27&31,063.39\\
&Var.&5,502.56&2.21&1,117.67&25.42&0.02&0.04&1,006.86&3,161.10&6,089.05&5,376.17&0.00&107,601,074.84&1,493,941,874.59&965,228,448.51\\\hline
\multirow{5}{*}{Poisoned (2\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&39.80&0.00&0.00&0.00&0.00&0.00&0.00&13,014.80\\
&Max&255.00&12.60&246.80&250.00&14.20&14.20&236.80&242.80&254.20&252.40&0.00&157,088.20&166,265.00&219,330.40\\
&Avg&66.53&1.00&15.84&0.95&0.01&0.01&221.95&199.10&121.87&99.29&0.00&884.51&67,140.64&44,139.47\\
&Std.&74.46&1.48&33.39&5.03&0.26&0.36&31.59&56.69&78.09&73.52&0.00&10,405.12&38,698.27&31,084.81\\
&Var.&5,544.98&2.20&1,114.62&25.34&0.07&0.14&998.16&3,217.26&6,097.91&5,405.39&0.00&108,274,860.43&1,497,572,415.35&966,492,706.86\\\hline
\multirow{5}{*}{Poisoned (3\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&29.00&0.00&0.00&0.00&0.00&0.00&0.00&13,107.60\\
&Max&255.00&12.40&247.60&250.60&19.40&19.40&232.20&248.40&254.60&254.40&0.00&157,013.00&165,769.20&219,365.60\\
&Avg&66.80&1.00&15.84&0.95&0.01&0.02&221.60&199.62&120.22&99.54&0.00&884.76&67,315.36&44,370.52\\
&Std.&74.59&1.48&33.36&5.03&0.35&0.49&32.59&55.84&77.98&73.85&0.00&10,408.17&38,769.05&31,105.51\\
&Var.&5,563.69&2.19&1,113.33&25.31&0.12&0.25&1,067.54&3,120.00&6,081.02&5,454.05&0.00&108,343,407.02&1,503,074,952.94&967,802,481.63\\\hline
\multirow{5}{*}{Poisoned (5\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&37.40&0.00&0.00&0.00&0.00&0.00&0.00&13,287.00\\
&Max&255.00&12.60&251.60&251.60&33.80&33.80&236.80&250.40&254.00&251.00&0.00&157,542.00&165,957.00&219,490.60\\
&Avg&67.47&1.00&15.84&0.96&0.02&0.03&221.95&200.22&120.06&98.56&0.00&884.75&67,454.62&44,604.35\\
&Std.&75.04&1.48&33.32&5.02&0.60&0.85&31.63&54.67&78.09&73.80&0.00&10,411.69&38,850.89&31,050.17\\
&Var.&5,631.69&2.18&1,110.46&25.22&0.36&0.72&1,000.80&2,989.46&6,098.53&5,446.95&0.00&108,411,860.17&1,509,414,001.41&964,216,169.73\\\hline
\multirow{5}{*}{Poisoned (7\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&36.60&0.00&0.00&0.00&0.00&0.00&0.00&13,354.40\\
&Max&255.00&12.00&251.60&251.60&44.60&44.60&234.00&250.00&253.00&249.40&0.00&158,001.20&164,868.60&219,529.60\\
&Avg&67.28&1.00&15.77&0.95&0.02&0.04&221.95&200.15&119.81&99.07&0.00&883.06&67,504.58&44,903.65\\
&Std.&74.66&1.47&33.07&5.00&0.79&1.12&31.49&54.36&77.89&74.61&0.00&10,398.90&38,915.47&30,965.77\\
&Var.&5,574.99&2.16&1,093.31&25.00&0.63&1.27&991.53&2,958.31&6,066.68&5,566.59&0.00&108,140,018.32&1,514,457,585.90&959,411,911.60\\\hline
\multirow{5}{*}{Poisoned (10\%)}&Min&0.00&0.00&0.00&0.00&0.00&0.00&35.40&0.00&0.00&0.00&0.00&0.00&0.00&13,404.20\\
&Max&255.00&12.00&247.40&247.40&64.60&64.60&234.20&246.80&254.40&249.80&0.00&155,748.20&162,128.00&217,657.80\\
&Avg&68.33&1.00&15.74&0.95&0.03&0.07&221.95&199.37&118.89&95.75&0.00&878.16&67,644.00&45,336.55\\
&Std.&75.30&1.46&32.92&4.98&1.15&1.63&31.16&54.54&78.35&73.83&0.00&10,327.47&38,962.82&30,707.17\\
&Var.&5,669.85&2.15&1,084.01&24.84&1.33&2.66&971.28&2,975.74&6,139.18&5,452.29&0.00&106,676,969.06&1,518,177,548.27&943,247,524.91\\\hline
\end{tabular}
}
\end{table*}

==> tables/results/adversarial0.01.tex <==

\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Adversarial (Epsilon 0.01)}
\label{tab:results-adversarial0.01}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline


Clean&98.22&90.26&45.29&44.30&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.27&50.75\\\hline
Adversarial (1\%)&98.18&90.26&45.30&44.30&6.25&0.10&0.12&98.65&97.30&90.33&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.04&0.00&0.01&0.00&0.00&0.00&0.00&0.00&0.00&-0.07&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.00&0.14&0.00&0.00&0.00&0.00&0.00&0.00&-0.54&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (2\%)&98.16&90.16&45.28&44.26&6.25&0.11&0.15&98.65&97.30&90.27&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.06&-0.09&-0.01&-0.04&0.00&0.01&0.03&0.00&0.00&-0.13&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&-0.31&-0.14&-0.36&0.00&0.20&0.38&0.00&0.00&-1.00&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (3\%)&98.24&90.36&45.30&44.30&6.26&0.10&0.12&98.65&97.30&90.27&45.27&0.00&1.49&21.34&50.75\\
Difference &0.02&0.11&0.00&0.00&0.00&0.00&0.00&0.00&0.00&-0.13&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.38&0.00&0.00&0.00&0.00&0.00&0.00&0.00&-1.00&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (5\%)&98.06&90.28&45.31&44.32&6.26&0.11&0.15&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.16&0.03&0.02&0.03&0.01&0.01&0.03&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.10&0.29&0.27&1.00&0.20&0.38&0.00&0.00&0.00&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (7\%)&98.00&90.34&45.25&44.35&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.22&0.08&-0.04&0.05&0.00&-0.01&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.28&-0.57&0.45&0.00&-0.20&0.00&0.00&0.00&0.00&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (10\%)&98.18&90.46&45.32&44.36&6.25&0.14&0.20&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.04&0.20&0.03&0.07&0.00&0.04&0.08&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.69&0.43&0.64&0.00&0.80&1.00&0.00&0.00&0.00&0.00&0.00&0.00&1.00&0.00\\\hline

\end{tabular}
}
\end{table*}


==> tables/results/adversarial0.05.tex <==


\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Adversarial (Epsilon 0.05)}
\label{tab:results-adversarial0.05}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
Clean&98.22&90.26&45.29&44.30&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.27&50.75\\\hline
Adversarial (1\%)&97.52&90.53&45.31&44.31&6.25&0.21&0.33&98.65&97.30&90.27&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.70&0.27&0.02&0.01&0.00&0.11&0.21&0.00&0.00&-0.14&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.28&0.06&0.06&0.00&0.22&0.21&0.00&0.00&-0.34&0.00&0.00&0.00&0.32&0.00\\\hline
Adversarial (2\%)&96.70&90.64&45.36&44.28&6.25&0.23&0.38&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-1.52&0.38&0.07&-0.01&0.00&0.13&0.26&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.40&0.22&-0.06&0.00&0.26&0.26&0.00&0.00&0.00&0.00&0.00&0.00&0.32&0.00\\\hline
Adversarial (3\%)&96.32&90.78&45.44&44.31&6.26&0.33&0.56&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-1.90&0.53&0.14&0.01&0.01&0.22&0.44&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.55&0.44&0.06&0.50&0.44&0.44&0.00&0.00&0.00&0.00&0.00&0.00&0.32&0.00\\\hline
Adversarial (5\%)&94.70&90.84&45.46&44.40&6.26&0.35&0.61&98.65&97.30&90.00&45.27&0.00&1.49&21.34&50.75\\
Difference &-3.52&0.58&0.17&0.10&0.01&0.25&0.49&0.00&0.00&-0.41&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.60&0.53&0.63&0.50&0.50&0.49&0.00&0.00&-1.00&0.00&0.00&0.00&0.32&0.00\\\hline
Adversarial (7\%)&93.38&91.22&45.57&44.42&6.27&0.51&0.91&98.65&97.43&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-4.84&0.96&0.28&0.12&0.02&0.41&0.79&0.00&0.13&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&1.00&0.88&0.75&1.00&0.82&0.79&0.00&1.00&0.00&0.00&0.00&0.00&0.32&0.00\\\hline
Adversarial (10\%)&90.98&90.89&45.61&44.45&6.27&0.60&1.12&98.65&97.43&90.27&45.27&0.00&1.49&21.49&50.75\\
Difference &-7.24&0.63&0.32&0.15&0.01&0.50&1.00&0.00&0.13&-0.14&0.00&0.00&0.00&0.22&0.00\\
Normalized Diff&N/A&0.66&1.00&0.94&0.50&1.00&1.00&0.00&1.00&-0.34&0.00&0.00&0.00&1.00&0.00\\\hline
\end{tabular}
}
\end{table*}


==> tables/results/adversarial0.10.tex <==


\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Adversarial (Epsilon 0.1)}
\label{tab:results-adversarial0.10}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
Clean&98.22&90.26&45.29&44.30&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.27&50.75\\\hline
Adversarial (1\%)&97.26&91.43&45.43&44.36&6.26&0.87&1.57&98.65&97.30&90.41&45.27&0.00&1.49&21.34&50.75\\
Difference &-0.96&1.17&0.14&0.07&0.01&0.77&1.45&0.00&0.00&0.00&0.00&0.00&0.00&0.07&0.00\\
Normalized Diff&N/A&0.55&0.12&0.16&0.09&0.29&0.29&0.00&0.00&0.00&0.00&0.00&0.00&0.10&0.00\\\hline
Adversarial (2\%)&96.30&91.74&45.58&44.43&6.28&1.10&2.00&98.65&97.30&90.41&45.27&0.00&1.49&21.42&50.75\\
Difference &-1.92&1.48&0.29&0.14&0.02&1.00&1.88&0.00&0.00&0.00&0.00&0.00&0.00&0.15&0.00\\
Normalized Diff&N/A&0.70&0.25&0.32&0.18&0.37&0.38&0.00&0.00&0.00&0.00&0.00&0.00&0.22&0.00\\\hline
Adversarial (3\%)&95.32&92.03&45.70&44.46&6.29&1.26&2.32&98.65&97.30&90.41&45.27&0.00&1.49&21.49&50.75\\
Difference &-2.90&1.77&0.41&0.16&0.03&1.16&2.20&0.00&0.00&0.00&0.00&0.00&0.00&0.22&0.00\\
Normalized Diff&N/A&0.83&0.35&0.36&0.27&0.43&0.45&0.00&0.00&0.00&0.00&0.00&0.00&0.33&0.00\\\hline
Adversarial (5\%)&93.40&92.18&45.98&44.58&6.31&1.85&3.32&98.65&97.30&90.41&45.27&0.00&1.49&21.79&50.75\\
Difference &-4.82&1.92&0.68&0.28&0.06&1.75&3.20&0.00&0.00&0.00&0.00&0.00&0.00&0.52&0.00\\
Normalized Diff&N/A&0.91&0.59&0.64&0.55&0.66&0.65&0.00&0.00&0.00&0.00&0.00&0.00&0.78&0.00\\\hline
Adversarial (7\%)&91.64&92.38&46.20&44.74&6.33&2.29&4.25&98.65&97.43&90.94&45.27&0.00&1.49&21.94&50.75\\
Difference &-6.58&2.12&0.91&0.44&0.07&2.18&4.13&0.00&0.13&0.54&0.00&0.00&0.00&0.67&0.00\\
Normalized Diff&N/A&1.00&0.78&1.00&0.64&0.82&0.84&0.00&1.00&0.79&0.00&0.00&0.00&1.00&0.00\\\hline
Adversarial (10\%)&88.52&92.34&46.45&44.70&6.36&2.77&5.05&98.65&97.43&90.27&45.27&0.00&1.49&21.71&50.75\\
Difference &-9.70&2.08&1.16&0.40&0.11&2.67&4.93&0.00&0.13&-0.14&0.00&0.00&0.00&0.44&0.00\\
Normalized Diff&N/A&0.98&1.00&0.91&1.00&1.00&1.00&0.00&1.00&-0.21&0.00&0.00&0.00&0.66&0.00\\\hline
\end{tabular}
}
\end{table*}


==> tables/results/adversarial0.20.tex <==


\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Adversarial (Epsilon 0.2)}
\label{tab:results-adversarial0.20}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
Clean&98.22&90.26&45.29&44.30&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.27&50.75\\\hline
Adversarial (1\%)&97.22&92.09&45.49&44.47&6.30&1.90&3.38&98.65&97.30&90.41&45.27&0.00&1.49&21.71&50.75\\
Difference &-1.00&1.84&0.20&0.17&0.05&1.80&3.26&0.00&0.00&0.00&0.00&0.00&0.00&0.44&0.00\\
Normalized Diff&N/A&0.64&0.12&0.18&0.17&0.34&0.34&0.00&0.00&0.00&0.00&0.00&0.00&0.13&0.00\\\hline
Adversarial (2\%)&96.22&92.51&45.69&44.51&6.33&2.30&4.06&98.65&97.30&90.41&45.27&0.04&1.57&22.31&50.75\\
Difference &-2.00&2.25&0.40&0.21&0.08&2.19&3.94&0.00&0.00&0.00&0.00&0.04&0.08&1.04&0.00\\
Normalized Diff&N/A&0.78&0.24&0.22&0.28&0.41&0.41&0.00&0.00&0.00&0.00&0.13&0.21&0.30&0.00\\\hline
Adversarial (3\%)&95.24&92.69&45.87&44.59&6.37&3.08&5.55&98.65&97.30&90.27&45.27&0.15&1.72&23.06&50.75\\
Difference &-2.98&2.43&0.58&0.30&0.12&2.98&5.43&0.00&0.00&-0.14&0.00&0.15&0.23&1.79&0.00\\
Normalized Diff&N/A&0.84&0.34&0.31&0.41&0.56&0.56&0.00&0.00&-1.00&0.00&0.50&0.61&0.51&0.00\\\hline
Adversarial (5\%)&93.38&92.77&46.23&44.78&6.42&3.79&6.66&98.65&97.43&90.27&45.27&0.19&1.87&24.18&50.75\\
Difference &-4.84&2.51&0.93&0.48&0.17&3.69&6.54&0.00&0.13&-0.14&0.00&0.19&0.38&2.91&0.00\\
Normalized Diff&N/A&0.87&0.55&0.49&0.59&0.69&0.68&0.00&1.00&-1.00&0.00&0.63&1.00&0.83&0.00\\\hline
Adversarial (7\%)&91.40&93.01&46.58&45.04&6.48&4.43&7.80&98.65&97.30&90.41&45.27&0.30&1.87&24.26&50.75\\
Difference &-6.82&2.76&1.29&0.74&0.23&4.33&7.68&0.00&0.00&0.00&0.00&0.30&0.38&2.99&0.00\\
Normalized Diff&N/A&0.96&0.76&0.76&0.79&0.81&0.80&0.00&0.00&0.00&0.00&1.00&1.00&0.85&0.00\\\hline
Adversarial (10\%)&88.34&93.14&46.99&45.27&6.55&5.46&9.77&98.65&97.30&90.41&45.27&0.30&1.87&24.78&50.75\\
Difference &-9.88&2.88&1.70&0.97&0.29&5.35&9.65&0.00&0.00&0.00&0.00&0.30&0.38&3.51&0.00\\
Normalized Diff&N/A&1.00&1.00&1.00&1.00&1.00&1.00&0.00&0.00&0.00&0.00&1.00&1.00&1.00&0.00\\\hline
\end{tabular}
}
\end{table*}


==> tables/results/adversarial0.30.tex <==


\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Adversarial (Epsilon 0.3)}
\label{tab:results-adversarial0.30}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
Clean&98.22&90.26&45.29&44.30&6.25&0.10&0.12&98.65&97.30&90.41&45.27&0.00&1.49&21.27&50.75\\\hline
Adversarial (1\%)&97.26&92.06&45.50&44.43&6.30&1.81&3.21&98.65&97.30&90.41&45.27&0.15&1.72&22.28&50.75\\
Difference &-0.96&1.80&0.20&0.13&0.04&1.70&3.09&0.00&0.00&0.00&0.00&0.15&0.23&1.01&0.00\\
Normalized Diff&N/A&0.58&0.11&0.13&0.13&0.31&0.31&0.00&0.00&0.00&0.00&0.50&0.61&0.29&0.00\\\hline
Adversarial (2\%)&96.26&92.66&45.70&44.73&6.34&2.58&4.50&98.65&97.30&90.41&45.27&0.23&1.87&22.61&50.75\\
Difference &-1.96&2.41&0.41&0.43&0.09&2.48&4.38&0.00&0.00&0.00&0.00&0.23&0.38&1.34&0.00\\
Normalized Diff&N/A&0.78&0.23&0.43&0.28&0.45&0.44&0.00&0.00&0.00&0.00&0.77&1.00&0.38&0.00\\\hline
Adversarial (3\%)&95.32&92.85&45.89&44.81&6.38&3.07&5.55&98.65&97.30&90.41&45.27&0.23&1.87&23.21&50.75\\
Difference &-2.90&2.60&0.60&0.51&0.12&2.96&5.43&0.00&0.00&0.00&0.00&0.23&0.38&1.94&0.00\\
Normalized Diff&N/A&0.84&0.34&0.50&0.38&0.53&0.55&0.00&0.00&0.00&0.00&0.77&1.00&0.55&0.00\\\hline
Adversarial (5\%)&93.42&93.19&46.31&44.95&6.45&3.79&6.67&98.65&97.30&90.41&45.27&0.26&1.87&23.28&50.75\\
Difference &-4.80&2.93&1.02&0.65&0.20&3.69&6.55&0.00&0.00&0.00&0.00&0.26&0.38&2.01&0.00\\
Normalized Diff&N/A&0.95&0.58&0.64&0.63&0.66&0.66&0.00&0.00&0.00&0.00&0.87&1.00&0.57&0.00\\\hline
Adversarial (7\%)&91.40&93.34&46.67&45.14&6.51&4.67&8.12&98.65&97.30&90.41&45.27&0.30&1.87&24.48&50.75\\
Difference &-6.82&3.08&1.37&0.84&0.25&4.57&8.00&0.00&0.00&0.00&0.00&0.30&0.38&3.21&0.00\\
Normalized Diff&N/A&1.00&0.78&0.83&0.78&0.82&0.81&0.00&0.00&0.00&0.00&1.00&1.00&0.91&0.00\\\hline
Adversarial (10\%)&88.50&93.35&47.06&45.31&6.57&5.66&9.99&98.65&97.30&90.95&45.27&0.30&1.87&24.78&50.75\\
Difference &-9.72&3.09&1.76&1.01&0.32&5.56&9.87&0.00&0.00&0.54&0.00&0.30&0.38&3.51&0.00\\
Normalized Diff&N/A&1.00&1.00&1.00&1.00&1.00&1.00&0.00&0.00&1.00&0.00&1.00&1.00&1.00&0.00\\\hline
\end{tabular}
}
\end{table*}



==> tables/results/functional.tex <==



\begin{table*}[t]
	\centering
	\caption{Functional Diversity Results for MNIST}
\label{tab:results-functional}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
1 Label&97.00&63.55&28.68&34.85&6.46&0.05&0.08&100.00&98.65&92.30&72.57&0.00&0.00&75.23&99.70\\\hline
2 Label&97.48&76.27&35.83&45.84&7.45&0.09&0.12&100.00&99.05&95.14&78.11&0.00&0.00&79.85&100.00\\
Difference &0.47&12.72&7.15&10.99&0.99&0.04&0.04&0.00&0.40&2.84&5.54&0.00&0.00&4.62&0.30\\
Normalized Diff&N/A&0.49&0.61&0.43&0.52&0.57&0.80&0.00&0.60&0.62&0.71&0.00&0.00&0.76&1.00\\\hline
3 Label&95.93&79.74&37.11&51.12&7.80&0.08&0.08&100.00&99.05&95.54&79.33&0.00&0.00&81.04&100.00\\
Difference &-1.08&16.19&8.43&16.27&1.34&0.02&0.00&0.00&0.40&3.24&6.76&0.00&0.00&5.82&0.30\\
Normalized Diff&N/A&0.62&0.72&0.64&0.70&0.29&0.00&0.00&0.60&0.71&0.86&0.00&0.00&0.95&1.00\\\hline
5 Label&96.30&85.13&39.16&57.74&8.15&0.11&0.10&100.00&99.32&96.08&79.46&0.00&0.00&81.19&100.00\\
Difference &-0.70&21.58&10.48&22.89&1.70&0.06&0.01&0.00&0.67&3.78&6.89&0.00&0.00&5.97&0.30\\
Normalized Diff&N/A&0.83&0.89&0.89&0.89&0.86&0.20&0.00&1.00&0.82&0.88&0.00&0.00&0.98&1.00\\\hline
7 Label&96.65&87.32&39.89&58.54&8.25&0.10&0.12&100.00&99.05&96.49&80.27&0.00&0.00&81.34&100.00\\
Difference &-0.35&23.77&11.21&23.69&1.79&0.04&0.04&0.00&0.40&4.19&7.70&0.00&0.00&6.11&0.30\\
Normalized Diff&N/A&0.91&0.95&0.93&0.94&0.57&0.80&0.00&0.60&0.91&0.98&0.00&0.00&1.00&1.00\\\hline
10 Labels&96.60&89.68&40.42&60.45&8.37&0.13&0.13&100.00&99.32&96.89&80.41&0.00&0.00&81.34&100.00\\
Difference &-0.40&26.12&11.74&25.60&1.91&0.07&0.05&0.00&0.67&4.59&7.84&0.00&0.00&6.11&0.30\\
Normalized Diff&N/A&1.00&1.00&1.00&1.00&1.00&1.00&0.00&1.00&1.00&1.00&0.00&0.00&1.00&1.00\\\hline
\end{tabular}
}
\end{table*}


==> tables/results/poisoned.tex <==

\begin{table*}[t]
	\centering
	\caption{Defect Detection Results for MNIST-Poisoned}
\label{tab:results-poisoned}
\scalebox{0.8}{\begin{tabular}{|L{2.2cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{0.8cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|R{1.0cm}|}
		 \hline
		   	    \textbf{}  &  \textbf{Acc}&  \textbf{KMNC (10)} & \textbf{KMNC (1000)} &\textbf{TKNC (10)}&\textbf{TKNC (1000)}  & \textbf{NBC} & \textbf{SNAC}  & \textbf{NC (0)} & \textbf{NC (0.2)} &\textbf{NC (0.5)} &\textbf{NC (0.75)} &\textbf{MC/DC (SS)}& \textbf{MC/DC (SV)}& \textbf{MC/DC (VS)}& \textbf{MC/DC (VV)}\\
		   	    \hline
Clean&98.52&89.12&43.95&76.18&9.76&0.14&0.12&100.00&97.57&97.30&81.35&0.00&0.75&84.70&100.00\\\hline
Poisoned (1\%)&97.70&89.59&44.04&76.23&9.77&0.32&0.39&100.00&97.57&97.16&81.35&0.00&0.75&84.70&100.00\\
Difference &-0.82&0.47&0.09&0.05&0.01&0.18&0.27&0.00&0.00&-0.14&0.00&0.00&0.00&0.00&0.00\\
Normalized Diff&N/A&0.27&0.12&0.19&0.33&0.17&0.21&0.00&0.00&-1.00&0.00&0.00&0.00&0.00&0.00\\\hline
Poisoned (2\%)&96.74&89.87&44.13&76.10&9.77&0.49&0.57&100.00&97.57&97.30&81.35&0.00&0.75&84.55&100.00\\
Difference &-1.78&0.75&0.18&-0.08&0.01&0.35&0.44&0.00&0.00&0.00&0.00&0.00&0.00&-0.15&0.00\\
Normalized Diff&N/A&0.43&0.23&-0.30&0.33&0.34&0.34&0.00&0.00&0.00&0.00&0.00&0.00&-0.33&0.00\\\hline
Poisoned (3\%)&95.76&90.19&44.23&76.23&9.77&0.57&0.78&100.00&97.57&97.30&81.35&0.00&0.75&84.70&100.00\\
Difference &-2.76&1.07&0.28&0.05&0.02&0.44&0.65&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
Normalized Diff&N/A&0.62&0.36&0.19&0.67&0.43&0.50&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\\hline
Poisoned (5\%)&93.96&90.47&44.36&76.12&9.78&0.77&0.86&100.00&97.57&97.30&81.35&0.00&0.75&84.85&100.00\\
Difference &-4.56&1.35&0.41&-0.06&0.03&0.63&0.74&0.00&0.00&0.00&0.00&0.00&0.00&0.15&0.00\\
Normalized Diff&N/A&0.78&0.53&-0.22&1.00&0.61&0.57&0.00&0.00&0.00&0.00&0.00&0.00&0.33&0.00\\\hline
Poisoned (7\%)&92.32&90.51&44.49&76.23&9.78&1.01&1.32&100.00&97.57&97.30&81.35&0.00&0.60&85.00&100.00\\
Difference &-6.20&1.39&0.54&0.05&0.03&0.87&1.20&0.00&0.00&0.00&0.00&0.00&-0.15&0.30&0.00\\
Normalized Diff&N/A&0.80&0.70&0.19&1.00&0.84&0.92&0.00&0.00&0.00&0.00&0.00&-1.00&0.67&0.00\\\hline
Poisoned (10\%)&89.60&90.85&44.72&75.96&9.79&1.17&1.43&100.00&97.57&97.30&81.35&0.00&0.75&84.70&100.00\\
Difference &-8.92&1.73&0.77&-0.22&0.03&1.03&1.30&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\
Normalized Diff&N/A&1.00&1.00&-0.81&1.00&1.00&1.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00&0.00\\\hline



\end{tabular}
}
\end{table*}

